A Balanced Data Approach for Evaluating Cross-Lingual Transfer: Mapping the Linguistic Blood Bank

We show that the choice of pretraining languages affects downstream cross-lingual transfer for BERT-based models. We inspect zero-shot performance in balanced data conditions to mitigate data size confounds, classifying pretraining languages that improve downstream performance as donors, and languages that are improved in zero-shot performance as recipients. We develop a method of quadratic time complexity in the number of languages to estimate these relations, instead of an exponential exhaustive computation of all possible combinations. We find that our method is effective on a diverse set of languages spanning different linguistic features and two downstream tasks. Our findings can inform developers of large-scale multilingual language models in choosing better pretraining configurations.

==> tables/cont.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table*}[tb!]
\small
\centering
\begin{tabular}{@{}cccccccccccccc@{}}
\textbf{ne}                           & \textbf{hi}                           & \textbf{de}                           & \textbf{hu}                           & \textbf{en}                           & \textbf{he}                           & \textbf{hy}                           & \textbf{ja}                                                  & \textbf{pms}                                                 & \textbf{ru}                                                  & \textbf{ta}                                                   & \textbf{fi}                                                   & \textbf{el}                                                   & \textbf{ar}                                                   \\
\cellcolor[HTML]{FFFFFF}\textbf{8.16} & \cellcolor[HTML]{FFFFC7}\textbf{7.79} & \cellcolor[HTML]{FFFC9E}\textbf{5.66} & \cellcolor[HTML]{FFCC67}\textbf{4.82} & \cellcolor[HTML]{FFCB2F}\textbf{3.88} & \cellcolor[HTML]{FFC702}\textbf{3.38} & \cellcolor[HTML]{F56B00}\textbf{2.33} & \cellcolor[HTML]{CB0000}{\color[HTML]{FFFFFF} \textbf{0.67}} & \cellcolor[HTML]{CB0000}{\color[HTML]{FFFFFF} \textbf{0.50}} & \cellcolor[HTML]{9A0000}{\color[HTML]{FFFFFF} \textbf{-1.0}} & \cellcolor[HTML]{680100}{\color[HTML]{FFFFFF} \textbf{-1.25}} & \cellcolor[HTML]{330001}{\color[HTML]{FFFFFF} \textbf{-2.25}} & \cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{-2.96}} & \cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{-3.81}}
\end{tabular}
\caption{Wasserstein distance means and standard deviation for all available data against our smaller datasets, over all languages. We created length distribution for sentences and words in both our training data and the full data as compared them using Earth Movers Distance (Wasserstein). Sentence length was truncated to 128 as in the training procedure (note that a sentence with 128 words is guarantied to have $\geq$ 128 tokens, meaning we overestimate).}
\label{tab:cont}
\end{table*}

==> tables/distance_stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table*}[tb!]
\small
\centering
\begin{tabular}{@{}lll@{}}
\toprule
                                    & \multicolumn{1}{c}{\textbf{mean}} & \multicolumn{1}{c}{\textbf{std}} \\ \midrule
\textbf{Sentence lengths in words}  & 0.0001                            & 2.445e-05                        \\
\textbf{Sentence lengths in tokens} & 0.0001                            & 1.870e-05                        \\
\textbf{Word Lengths}               & 1.645e-05                         & 6.708e-06                        \\ \midrule
                                    &                                   &                                 
\end{tabular}
\caption{Wasserstein distance means and standard deviation for all available data against our smaller datasets, over all languages. We created length distribution for sentences and words in both our training data and the full data as compared them using Earth Movers Distance (Wasserstein). Sentence length was truncated to 128 as in the training procedure (note that a sentence with 128 words is guarantied to have $\geq$ 128 tokens, meaning we overestimate).}
\label{tab:data_dists}
\end{table*}

==> tables/lang_choice_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table*}[tb!]
\small
\centering
\begin{tabular}{@{}ccccccccccccccccccccccc@{}}
\toprule
               & \textbf{Ja} & \textbf{Ko} & \textbf{Ta}   & \textbf{Te}   & \textbf{Hu}  & \textbf{Fi} & \textbf{Zh}     & \textbf{My}    & \textbf{Ar}  & \textbf{He}  & \textbf{Cy}  & \textbf{Ga} & \textbf{Hi}    & \textbf{Ne}   & \textbf{En}   & \textbf{De}  & \textbf{Hy}       & \textbf{El}      & \textbf{Fr}  & \textbf{Pmd} & \textbf{Ru}  & \textbf{Sv} \\ \midrule
Relation       & \multicolumn{2}{c}{-}     & \multicolumn{2}{c}{Dravidian} & \multicolumn{2}{c}{Uralic} & \multicolumn{2}{c}{Sino-Tibetan} & \multicolumn{2}{c}{Semitic} & \multicolumn{2}{c}{Celtic} & \multicolumn{2}{c}{Indo-Aryan} & \multicolumn{2}{c}{Germanic} & \multicolumn{2}{c}{remotely related} & \multicolumn{2}{c}{Romance} & \multicolumn{2}{c}{slavic} \\
Share alphabet & \multicolumn{2}{c}{No}    & \multicolumn{2}{c}{No}        & \multicolumn{2}{c}{Yes}    & \multicolumn{2}{c}{No}           & \multicolumn{2}{c}{No}      & \multicolumn{2}{c}{Yes}    & \multicolumn{2}{c}{Yes}        & \multicolumn{2}{c}{Yes}      & \multicolumn{2}{c}{No}               & \multicolumn{2}{c}{Yes}     & \multicolumn{2}{c}{No}     \\ \bottomrule
\end{tabular}
\caption{Chosen Language couples for analysis. Notice that some languages share alphabets (e.g. German and English) and others do not (e.g. Hebrew and Arabic). This gives us a possibility to see if non-alphabetic relations are captured. Japanese and Korean were clustered together although they correspond to singleton families. }
\label{tab:lang-choice}
\end{table*}

==> tables/main-results-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table*}[tb!]
\small
\centering
\begin{tabular}{@{}llllllll@{}}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Diag avg.}} & \multirow{2}{*}{\textbf{0 shot avg}} & \multicolumn{2}{l}{\textbf{Most cont}} & \multicolumn{2}{l}{\textbf{Least cont avg.}} & \multirow{2}{*}{\textbf{Zero shot for pretrain}} \\
                  &                                     &                                      & \textbf{0 shot}     & \textbf{eval}    & \textbf{0 shot}        & \textbf{eval}       &                                                  \\ \midrule
\textbf{Top}      & 0.571                               &                                      &                     &                  &                        &                     &                                                  \\
\textbf{Random}   &                                     &                                      &                     &                  &                        &                     &                                                  \\
\textbf{Bottom}   &                                     &                                      &                     &                  &                        &                     &                                                  \\ \bottomrule
\end{tabular}
\caption{Our main results table.}
\label{tab:main-results}
\end{table*}

==> tables/ner-results-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table*}[tb!]
\small
\centering
\begin{tabular}{llllllll}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{eval}} & \multirow{2}{*}{\textbf{0 shot}} & \multicolumn{2}{l}{\textbf{Most cont'}} & \multicolumn{2}{l}{\textbf{Least cont'}} & \multirow{2}{*}{\textbf{0 shot, pretrain set}} \\
                  &                                &                                  & \textbf{0 shot}     & \textbf{eval}     & \textbf{0 shot}      & \textbf{eval}     &                                                \\ \hline
\textbf{Top}      & \textbf{0.571}                 & \textbf{0.212}                   & \textbf{0.174}      & 0.566             & \textbf{0.118}       & 0.576             & \textbf{0.23}                                  \\
\textbf{Random}   & 0.331                          & 0.147                            & 0.125               & 0.333             & 0.080                & 0.330             & 0.192                                          \\
\textbf{Bottom}   & 0.320                          & 0.141                            & 0.096               & 0.329             & 0.010                & 0.312             & 0.16                                           \\
\textbf{Control}  & 0.331                          & 0.143                            & 0.120               & 0.330             & 0.078                & 0.333             & -                                             
\end{tabular}
\caption{NER results. We can see that the top influential configuration scores the best score in regular evaluation and zeroshot evaluation. Also, least contributed languages constantly under-perform contributed languages.}
\label{tab:ner-results}
\end{table*}

==> tables/pos-results-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table*}[tb!]
\small
\centering
\begin{tabular}{lllllll}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{eval}} & \multirow{2}{*}{\textbf{0 shot}} & \multicolumn{2}{l}{\textbf{Most cont'}} & \multicolumn{2}{l}{\textbf{Least cont'}} \\
                  &                                &                                  & \textbf{0 shot}     & \textbf{eval}     & \textbf{0 shot}      & \textbf{eval}     \\ \hline
\textbf{Top}      & \textbf{0.615}                 & \textbf{0.323}                   & \textbf{0.238}      & 0.64              & \textbf{0.21}        & 0.59              \\
\textbf{Random}   & 0.611                          & 0.319                            & \textbf{0.227}      & 0.626             & 0.205                & 0.583             \\
\textbf{Bottom}   & 0.618                          & 0.314                            & \textbf{0.224}      & 0.619             & 0.201                 & 0.59              \\
\textbf{Control}  & 0.618                          & 0.325                            & \textbf{0.238}      & 0.64              & 0.21                 & 0.596            
\end{tabular}
\caption{POS results. Although overall zeroshot and evaluation do not seem to be influenced by the pretrain set, most contributed languages constantly out do the least contributed ones in terms of zeroshot and evaluation.}
\label{tab:pos-results}
\end{table*}
